Unsupervised Visual Attribute Transfer with Reconfigurable Generative Adversarial Networks

Learning to transfer visual attributes requires supervision dataset. Corresponding images with varying attribute values with the same identity are required for learning the transfer function. This largely limits their applications, because capturing them is often a difficult task. To address the issue, we propose an unsupervised method to learn to transfer visual attribute. The proposed method can learn the transfer function without any corresponding images. Inspecting visualization results from various unsupervised attribute transfer tasks, we verify the effectiveness of the proposed method.

==> text/abstract_v1.tex <==
\begin{abstract}
In representation learning, \textit{disentangled representations} are a set of factored codes in which salient high-level features of input data are separately encoded. With disentangled representations, we can build a conditional generative model in which a designated factor code can be adjusted for the corresponding change in generation. Very recently, researchers show a possibility that disentangled representations can be learned with a Generative Adversarial Net (GAN). We explore this direction even further by examining an alternative model leveraged by the adversarial learning paradigm. 
In this paper, we present \textit{CrisprGAN}, a conditional generative model that learns \textit{composable} disentangled representations with GANs. With CrisprGAN, we can explicitly specify factor codes to learn, and simultaneously control multiple factor codes for generation. Basically, CrisprGAN consists of a \textit{conversion-reversion autoencoder} and \textit{conversion GANs} for partial discrimination. The main idea is that GANs can be effectively used to learn disentangled codes by performing \textit{partial discrimination} between real and sample data. The partial discrimination can be done by a simple but effective trick called \textit{factor conversion}. Each neural network of CrisprGAN can be jointly trained with backpropagation. Our experiments demonstrate that CrisprGAN effectively generates samples by simultaneously controlling multiple factor codes and learned disentangled representations are effective for downstream tasks such as classification.
\end{abstract}

==> text/abstract_v2.tex <==
\begin{abstract}
%Complex translation (CT) is a technique to translate multiple elements in data simultaneously. For example, converting an image of smiling male person with black hair into non-smiling female person with blond hair is a CT. However, in order to train a CT model, we need to gather datasets that contain all the possible combinations of elements of interests, which is highly labor intensive. On the other hand, CT can be expressed as the combinations of multiple simple translations (ST). The previous example can be decomposed into translations of male to female, smiling to non-smiling, and black hair to blond hair translations. In this paper, we propose a method to train a CT model by using only unpaired ... 

% new rewrite JK
<GeneGAN: Multiplex Image Translation by CRISPR-inspired Feature Editing> \newline
An image can be described in many aspects: place, object, attributes, typically belonging to many different domains. We consider the problem of image translation involving multiple domain adaptations. As existing paired or unpaired image translation \cite{isola2017im2im,zhu17cycle,kim2017discogan} methods are typically limited to consider only two domains, enabling each multiplex translation scenario requires new model learning. Explosion of combinatorially many possible translation scenarios makes approaches based on existing methods impractical. In this work, we propose a scalable single-model method capable of handling arbitrarily many multiplex image translations. The key idea, biologically-inspired by genome editing based on CRISPR \cite{ran2013crispr}, is to represent an image with two separate vectors: a genotype vector (softly) encoding domain membership and a phenotype vector encoding individual characteristics. Editing a specified region of gene vector and regenerate the corresponding image results in a two-domain image translations where individual characteristics specific to the given image are preserved. It is demonstrated that multiplex translations can be easily synthesized by editing several regions simultaneously requiring no additional data collected specifically for each case.  

% Generating an image with a different gene vector  Gene vector indicates 

% CRISPR-like feature editing GAN-based method to 

% Complex trans 하고 싶다. 경우의 수가 많다. 그래서 데이터 없다. complex trans는 simple trans 조합이다. 그러면, 데이터 있고, DiscoGAN 하면 된다. 그런데 모델이 무한히 늘어난다. 그래서 한 모델로 모든 complex tans하는 방식을 제한한다.

% Other
<Multiplex Image Translation with Generative Adversarial Networks>\newline
This paper investigates \textit{multiplex image translation} which includes multiple simple translations from a source domain to a target domain. An image is typically affiliated with multiple domains. For example, an image of a woman with black hair belongs to two different domains. Therefore, it is natural to consider that multiple translations are performed to translate an image and to have an output image with multiple effects applied (e.g., a woman with black hair $\rightarrow$ a man with brown hair). However, multiplex image translation requires to build multiple translation models for each translation.\newline
In this paper, we present an \textit{all-in-one image translator} with which multiplex translation can be performed either sequentially or simultaneously without the need for building multiple models. We demonstrate that a single shared model can be built by using \textit{disentangled image representations} which consist of two separate codes: (1) uniqueness code and (2) factor codes. 
changes made in factor codes allow the single shared model to perform different translations. The proposed model is effectively trained with Generative Adversarial Networks. Our experiment results show that the proposed model can effectively perform multiplex translations.
\end{abstract}

==> text/complex_translation.tex <==
\begin{figure}[t]
  \begin{center}
  \centerline{\includegraphics[width=0.5\linewidth]{Figures/Figure001_Complex_Translation_v_0_0_2_2017_05_18}}
  \caption{Complex translation (To be replaced)}
  \label{fig:complex_trans}
  \end{center}
\end{figure}

\begin{figure}[t]
  \begin{center}
  \centerline{\includegraphics[width=\linewidth]{Figures/Figure008_CRISPR_Cut_v_0_0_1_2017_05_18}}
  \caption{CRISPR-like Feature Editing - 이미지 변경 필요(이전 버전 이미지)}
  \label{fig:complex_trans}
  \end{center}
\end{figure}
Complex translation is to map an input data and an output data by changing multiple attributes (e.g, gender and hair color). In this case, the translation can be considered as the mapping between \textit{composite domains} that are expressed by the Cartesian product of simple domains (e.g., (man, blond hair), (man, black hair), (woman, blond hair), and (woman, black hair)). Figure \ref{fig:complex_trans} shows an example of composite domains and complex translations between them. There are four composite domains $\{AJ, AK, BJ, BK\}$ and twelve complex translations between them. 

Basically, complex translation can be achieved by sequentially applying simple translations. For example, a complex translation $AJ \rightarrow BK$ can be performed by $f: A \rightarrow B \quad \textrm{and} \quad g: X \rightarrow Y$. This approach can be generalized by the following formula, given $a \in A$, $b \in B$, $j \in J$, and $k \in K$:
\begin{equation}
(f*g)(x_{a,j}) = (f(x_{a,j}), g(x_{a,j})) = x_{b,k}
\end{equation}

Simple translation is to map an input data from source domain $A$ to an output data from target domain $B$ with regards to single attributes. The simple translation can be learned by GAN-based models such as DiscoGAN \cite{kim2017discogan}. More specifically, DiscoGAN proposed a model that has two generators $G_{AB}$ and $G_{BA}$, and associated adversarial discriminators $D_{B}$ and $D_{A}$. $D_{B}$ promotes $G_{AB}$ to translate inputs from domain $A$ into outputs that are indistinguishable from domain $B$. $D_{A}$ does a similar job. In addition to this, to further constrain the model, the reconstruction loss $x_{a} \rightarrow G_{AB}(x_{a}) \rightarrow G_{BA}(G_{AB}(x_{a})) = x''_{a}$ was additionally introduced.

However, the number of translations grows exponentially with regards to the number of attributes of composite domains. To address this problem effectively, we present a method to learn composite domain distribution by using simple domain distributions learned by GANs. In the next section, we describe the method in detail.

==> text/composite_domain_distribution.tex <==
\begin{figure}[t]
  \begin{center}
  \centerline{\includegraphics[width=0.8\textwidth]{Figures/Figure003_Complex_translation_Sampling_Converting_v_0_0_1_2017_05_17}}
  \caption{(a) : Simple Translation Success, (b) : Complex Translation Failure, (c) Complex Translation Success - XXXX Method -> AJ : Input, AK : Simple Translation Output, BK : Complex Translation Output}
  \label{fig:composite}
  \end{center}
\end{figure}

(TBD) \newline
$p_{g}(x|z,a) = G(z,b)$ and $D_{B}$ \newline
$p_{g}(x|z,k) = G(z,k)$ and $D_{K}$ \newline

We can induce $D_{BK}$ from $D_{B}$ and $D_{K}$.
$D_{B}$ promotes $G$ to learn $B$ distribution including both $B_{J}$ and $B_{K}$.
$D_{B}$ can promote $G$ to learn $BK$ distribution, when it see auxiliary sample $G(z,j)$ in addition to target sample $G(z,k)$.

Figure \ref{fig:composite} shows how to learn composite domain distribution. \newline
(TBD)

==> text/implementation.tex <==
\section{Implementation}

The implementation details of CrisprGAN is summarized in Table \ref{tab:imple}.

\begin{table}[b]
  \centering
  \caption{Network Architectures}   
  \label{tab:imple}
  \begin{tabular}{|l|l|l|}
  \hline
Encoder                                                                                                        & Generator (f=3)                                                                                                  & Discriminator                       \\ \hline
Input 128x128 Color Image                                                                                      & \begin{tabular}[c]{@{}l@{}}Input z: 32x32x256\\ Input f: 32x32x100 (fx100)\\ Concatenate: 32x32x526\end{tabular} & Input 128x128 Color Image           \\ \hline
7x7 Conv, 64 ReLU, BatchNorm                                                                                   & 7x7 Conv, 256 ReLU, BatchNorm                                                                                    & 4x4 Conv, 64 LeakyReLU, BatchNorm   \\ \hline
3x3 Conv, 128 ReLU, BatchNorm                                                                                  & \begin{tabular}[c]{@{}l@{}}{[}Residual{]}\\ 3x3 Conv, 256 ReLU, BatchNorm, \\ 3x3 Conv, BatchNorm\end{tabular}   & 4x4 Conv, 128 LeakyReLU, BatchNorm  \\ \hline
3x3 Conv, 256 ReLU, BatchNorm                                                                                  & \begin{tabular}[c]{@{}l@{}}{[}Residual{]}\\ 3x3 Conv, 256 ReLU, BatchNorm, \\ 3x3 Conv, BatchNorm\end{tabular}   & 4x4 Conv, 256 LeakyReLU, BatchNorm  \\ \hline
\begin{tabular}[c]{@{}l@{}}{[}Residual{]}\\ 3x3 Conv, 256 ReLU, BatchNorm, \\ 3x3 Conv, BatchNorm\end{tabular} & 3x3 Deconv, 128 ReLU, BatchNorm                                                                                  & 4x4 Conv, 512 LeakyReLU, BatchNorm  \\ \hline
                                                                                                               & 3x3 Deconv, 64 ReLU, BatchNorm                                                                                   & 4x4 Conv, 1024 LeakyReLU, BatchNorm \\ \hline
                                                                                                               & 7x7 Conv                                                                                                         & 4x4 Conv                            \\ \hline
                                                                 
  \end{tabular}
\end{table}

==> text/introduction_v1.tex <==
\section{Introduction}

Superdomain은 데이터를 설명할 수 있는 factor들 중 서로 independent하고, 동시에 우리가 관심을 갖고 있는 것들임. 여러 superdomain이 genotype vector의 영역을 나눠 차지하며, 각 superdomain은 복수 개의 domain으로 이뤄져 있음. 우리는 각 데이터 샘플을 unique 특징인 phenotype과, 여러 superdomain과 관련된 genotype으로 인코딩할 수 있으며, genotype의 특정 영역의 값을 바꾼 뒤 재생산해 의도했던 형질을 가진 새로운 데이터를 얻을 수 있다고 가정함. phenotype은 데이터의 unique한 특성이므로 genotype에 변경을 가하더라도 변하지 않으며, 이 논문에서는 각 task에서 정의한 superdomain들과 무관한 모든 특성을 phenotype이라고 한다. 예를 들어, 사람 얼굴 이미지와 관련된 superdomain으로서 성별과 머리 색깔을 정했다면, 얼굴형이나 피부색 등은 모두 phenotype이 된다. 
  
GeneGAN can perform \textit{multiplex translation}. Multiplex tanslation is to translate an input image in a source domain into an output image that can have multiple membership to many domains. For example, it can translate a face image with "blond hair" and "no-smile" into a face image with "black hair" and "smile", meantime other factors are kept intact. This multiplex translation is illustrated in Figure \ref{fig:multiplex}.

In GeneGAN, the translation mainly consists of three steps: (1) image encoding, (2) feature editing, and (3) image generation. GeneGAN first represents an input image with two separate vectors: (a) genotype vectors for domain membership and (b) a phenotype vector for indivisual characteristics. Then, GeneGAN edits a designated genotype vectors that induce the corresponding attribute changes in an output image. Finally, GeneGAN generates an output image from the edited vector representations. \ref{fig:multiplex} breifly illustrates such translation process.

To enable this kind of translation process, we presents a model that can learn the genotype and phenotype vector representations that induce the corresponding membership changes. The basic idea is that an adversarial discriminator of GAN can effectively used for checking the translated image is indistinguishable with images from the target domain. The details are provided in the following subsections. 
  
Unsupervised representation learning is one of most important reasons for the huge success of deep learning \cite{bengio2013deep}. It allows us to exploit a huge volume of unlabeled data for learning hidden representations that is useful for complex task with a small number of labeled data \cite{hinton2006rbm, hinton2006rbm2, vincent2008dae}. For some decades, there have been many research efforts such as restricted Boltzman machines (RBMs) \cite{hinton2006rbm,hinton2006rbm2} and Autoencoders (AEs) \cite{vincent2008dae} for the unsupervised representation learning. Recently, many researchers believe that good generative models such as Variational Autoencoders (VAEs) \cite{kingma2014vae} and Generative Adversarial Nets (GANs) \cite{goodfellow2014generative} will provide even better representations.

\textit{Disentangled representations} are a set of factored codes in which salient high-level features of input data are separately encoded \cite{bengio2013disrepre}. They allow us to build a conditional generative model in which a designated factored code is adjusted for the corresponding change in generation. Furthermore, they can be used for downstream machine learning tasks such as classifications, clustering, etc. Very recently, researchers show a possibility that disentangled representations can be learned with GANs. For example, Xi Chen et al. \cite{chen2016infogan} proposed InfoGAN, an extension of GAN with a variational regularization of mutual information. Michael Mathieu et al. \cite{mathieu2016cvaegan} proposed a conditional generative model based on VAE with extended by GAN. We explore this direction even further by examining an alternative model leveraged by the adversarial learning paradigm.

In this paper, We present \textit{CrisprGAN}, a conditional generative model that can learn \textit{composable} disentangled representations by exploiting GANs. One of main advantages of CrisprGAN is that we can disentangle composable factors by exploiting a large volume of weakly labeled data. For example, CrisprGAN allows us to collect face images with different hair colors (e.g., gold, brown, and black) regardless of gender and age in order to learn disentangled factor codes for the different hair colors of faces. In this manner, we can further compose desired factor codes that results in corresponding change in image generation. The main idea of CrisprGAN is that we can effectively use GANs for discriminating a part of data between real and sample (e.g., the hair color of a face) instead of discriminating the total data (e.g., a full face). For this purpose, we generate sample data which attributes are partially changed by replacing a designated factor code. We call this simple but effective trick \textit{factor conversion}. 

%(see Figure  \ref{fig:figure_1}).
% \begin{figure}[t]
%   \begin{center}
%   \centerline{\includegraphics[width=\textwidth]{Figures/followup_1}}
%   \caption{An example of CrisprGAN: Learning the disentangled representations for the hair color of faces}
%   \label{fig:figure_1}
%   \end{center}
% \end{figure} 

CrisprGAN consists of a \textit{conversion-reversion autoencoder} and \textit{conversion GANs} for partial discrimination. The conversion-reversion autoencoder is two autoencoder (i.e., conversion autoencoder and reversion autoencoder). It enables to learn the \textit{identify code} that captures the overall structure of data. And, the conversion GANs enable to learn the \textit{composable factor codes} that capture partial attributes of data (e.g., the hair color of a face). More specifically, the generator of the conversion GAN generates sample data that one of its attributes is partially changed by the factor conversion. Then, the discriminator of the conversion GAN examines whether the sample data generated with the factor conversion is real or not with regards to the specific attribute of data. Each neural network of CrisprGAN can be jointly trained with backpropagation.

We envision disentangled representations that are composable and editable. This concept is inspired by a genome editing tool called CRISPR \cite{ran2013crispr}. CRISPR makes it possible to correct mutations at precise locations in the human genome to treat genetic causes of disease. Composable disentangled representations can be considered as the counterpart with similar concept in machine learning. We investigate this direction little further with CrisprGAN, and believe that there will be much promising other research results in the research community.

Our experiments demonstrate that CrisprGAN effectively generates samples by simultaneously controlling multiple factor codes and learned disentangled representations are effective for downstream tasks such as classification. (TODO)

This paper is organized as follows. In Section 2, we provide the related work. In Section 3, we present the architecture and training method of CrisprGAN. Then, in Section 4, we describe the implementation details. The experiment results are presented in Section 5. And, we conclude this paper in Section 6.






==> text/introduction_v2.tex <==
\section{Introduction}
%% Key: 
There have been significant progress and increasing interest in the field of image stylization including image style transfer, texture transfer and color transfer \cite{colortransfer, styletransfer, texturetransfer}. These works all address the  visual attribute transfer problem, in which visual attributes of one image is copied over to the visual attributes of another image.  



% they are only capable of transferring the entire set of visual attributes and cannot select which attribute to copy over. For example, a color transfer network cannot selectively transfer the color at specific regions, and the same applies for style and texture transfer. 

%More recently, several methods succeeded in attribute level style transfer such as \cite{liao17transfer}. 
Despite the remarkable results of these works, most of these works are nonparametric exemplar-based. One reason for this can be that supervised learning of attribute level transfer with parametric model such as deep neural network requires paired data (two images that differ in only one attribute) that are nearly impossible to obtain. For example, in the case of transferring the gender attribute in face images, one would require images of each person in both male and female forms.   

% Such supervised data is seldom available and the cost of labeling can be high. In addition, it is difficult to pair the corresponding images when there are multiple close candidates. 

We therefore propose an unsupervised visual attribute transfer mechanism using controllable image translation networks. With our reconfigurable image translation framework, a single translation model can be easily reconfigured for various translation tasks each of which involve different visual attributes. 

Our image translation network uses the generative adversarial networks framework \cite{goodfellow2014generative} to learn to represent images as encodings of visual attributes. By changing the value of the encoding for an attribute to a desired target value, the input image can be selectively translated into an image of a different domain. Moreover, this translation network can be easily reconfigured to translate the input into different output domains by changing the target visual attribute and its desired value.

After training, the visual attribute of one image can be transfered to another image by replacing the encoded attribute value of one image with another and passing the new hybrid encoding through a generator network. 

We test our method on several visual attribute transfers: object angle and identity attributes, facial attributes, and fashion attributes. We empirically show that our  approach performs well on both reconfigurable image translation as well as visual attribute transfer. 
 
 
 
 
 
 
 
 
 
% 그래서 우리는 reconfigurable image translation을 이용해 이 문제를 풀었다 


%Our image translator is composed of two main operations: (1) \textit{translation} and (2)\textit{back-translation}. The neural network for translation can be effectively trained with Generative Adversarial Networks (GANs) \cite{goodfellow2014generative}. The adversarial discriminator $D$ of GAN encourages the generator $G$ to generate an output image with the desired image attribute,  ?? an indistinguishable one from the target domain's images. For this purpose, an adversarial objective called \textit{translation discrimination objective} is used. In addition to this, to maintain translation consistent, we use \textit{back-translation consistency objective}. This means that back-translated image should be mapped into to the original image. Recent research results \cite{kim2017discogan,zhu17cycle} demonstrated that such consistency loss significantly improves the image translation quality.   

%Comprehensive experiment results show that our all-in-one image translator can generate an high-quality output image where multiple changes (e.g., a smiling brown hair woman $\rightarrow$ a unsmiling black hair woman). This multiplex image translation can be performed sequentially and simultaneously.  

%This paper is structured as follows. We summarize the related works in section 2 and discuss relations and differences. In section 3, we present the architecture and training method of GeneGAN. Our experiment results are detailed in Section 4. We conclude the paper in section 5. 









%In computer vision and graphics, many problems can be conceptualized as image-to-image translation (e.g., labels to facade, day to night, face to car, etc.). The goal of image-to-image translation (or simply image translation) is to learn the mapping from an input image of source domain to the output image of target domain (i.e., $f : A \rightarrow B$). From the perspective of training, image translation can be categorized into two: (1) paired image  translation and (2) unpaired image translation. Paired image translation \cite{isola2017im2im} requires paired training data in the form of pairs of images $\{x_{i}, y_{i}\}$. However, obtaining paired training data is usually expensive. To address this issue, unpaired image-to-image translation \cite{kim2017discogan,zhu17cycle} has been proposed. This approach enables to learn the mapping between domains without paired input-output examples.

%However, an image is typically affiliated with multiple domains. For example, an image of a woman with black hair belongs to two domains (i.g., woman and black hair). Therefore, it is natural to consider that multiple translations are performed to translate an image and to have an output image with multiple effects applied (e.g., a woman with black hair $\rightarrow$ a man with brown hair). We call this \textit{multiplex image translation}. Conceptually, multiplex translation can be achieved by performing simple translation multiple times. However, this naive approach requires to build multiple translation models for each translation. Furthermore, as the number of affiliated domains increases, the number of possible translations increases exponentially. We need a sophisticated approach to address the model explosion.    

%In this paper, we propose an \textit{all-in-one image translator} with which multiplex translation can be performed either sequentially or simultaneously without the need for building multiple models. We demonstrate that the all-in-one image translator can be built by using \textit{disentangled image representations} \cite{bengio2013deep} which consist of two separate codes: (1) uniqueness code and (2) factor codes. Changes made in factor codes allow the all-in-one translator to perform different translations in a shared manner. 

%Our all-in-one image translator is composed of two main operations: (1) \textit{translation} and (2)\textit{back-translation}. The neural network for translation can be effectively trained with Generative Adversarial Networks (GANs) \cite{goodfellow2014generative}. The adversarial discriminator $D$ of GAN encourages the generator $G$ to generate a translated output image, an indistinguishable one from the target domain's images. For this purpose, an adversarial objective called \textit{translation discrimination objective} is used. In addition to this, to maintain translation consistent, we use \textit{back-translation consistency objective}. This means that back-translated image should be mapped into to the original image. Recent research results \cite{kim2017discogan,zhu17cycle} demonstrated that such consistency loss significantly improves the image translation quality.   

%Comprehensive experiment results show that our all-in-one image translator can generate an high-quality output image where multiple changes (e.g., a smiling brown hair woman $\rightarrow$ a unsmiling black hair woman). This multiplex image translation can be performed sequentially and simultaneously.  

%This paper is structured as follows. We summarize the related works in section 2 and discuss relations and differences. In section 3, we present the architecture and training method of GeneGAN. Our experiment results are detailed in Section 4. We conclude the paper in section 5.

==> text/model_v1.tex <==
\section{Model}
(This section is in a very early stage.)

In this section, we present the architecture and training method of CrisprGAN.

Some formula for conditional generative model. (TODO)

\begin{figure}[h!]
  \begin{center}
  \centerline{\includegraphics[width=\textwidth]{Figures/CrisprGAN_Architecture2}}
  \caption{The architecture of CrisprGAN}
  \label{fig:figure_2}
  \end{center}
\end{figure}

\subsection{Architecture}
Basically, CriprGAN consists of an stacked autoencoder and partial discrimination GANs. The architecture of CrisprGAN is shown in Figure \ref{fig:figure_2}. Basically, CriprGAN consists of an stacked autoencoder and partial discrimination GANs. The stacked autoencoder enables to learn the \textit{identify code} that captures the overall structure of data. And, the partial discrimination GANs enable to learn the \textit{composable factor codes} that capture partial attributes of data (e.g., the hair color of a face).

We start by describing the stacked autoencoder. The stacked autoencoder mainly consists of two sub autoencoders: Conversion Encoder-Decoder and Reversion Encoder-Decoder. Conversion Encoder-Decoder takes data x\textsubscript{a,b} with the factor \textit{a} and \textit{b} as input and generates sample data x’\textsubscript{a’,b} with a converted factor \textit{a’} and the same factor \textit{b}. It learns factored codes {z, a’, b} by converting a factor code a (i.e., factor conversion). Reversion Encoer-Decoder takes sample data x’\textsubscript{a’,b} with the converted factor \textit{a’} and the original factor \textit{b} as input and generates sample data x’\textsubscript{a,b} with the original factor \textit{a} and \textit{b}. It learns factored codes {z, a, b} by reverting a factor code a (called factor reversion). 

We note that Conversion Encoder and Reversion Encoder share their parameters. Conversion Decoder and Reversion Decoder share their parameters. More importantly, Conversion Decoder is shared with the Generator of partial discrimination GANs.

In CrisprGAN, Conversion GAN plays import role. The generator \textit{G} of Conversion GAN takes the converted codes {z, a’, b} as input, and generates a sample data x’\textsubscript{a’,b}. The discriminator \textit{D\textsubscript{a’}} of Conversion GAN takes a sample data \textit{x’\textsubscript{a’,b}} and a real data x\textsubscript{a’,b} as input, and generates the probability that the sample data came from the real dataset. The \textit{G} and D\textsubscript{a’} are trained simultaneously in a way of a minimax game with conversion GAN loss L\textsubscript{Da’}. 

In addition to Conversion GAN, we can use GAN for discriminating preserved factors. We call this auxiliary network Preservation GAN. Preservation GAN shares its generator \textit{G} with that of Conversion GAN. The discriminator D\textsubscript{b} of Preservation GAN takes a sample data x’\textsubscript{a’,b} and a real data x\textsubscript{a,b} as input, and generates the probability that the sample data came from the real dataset. The \textit{G} and D\textsubscript{b} are trained simultaneously in a way of a minimax game with preservation GAN loss L\textsubscript{Db}.


\subsection{Training}
Each neural network of CrisprGAN can be jointly trained with backpropagation. The loss function consists of mainly two terms: (1) the reconstruction loss of the autoencdoer and (2) the GAN loss for partial discrimination. 

%\subsection{Definitions}
%  우리는 데이터를 정의하는 많은 특징들 중, 다른 특징들과 완전히 구분되어 서로 영향을 끼지지 않는 특징을 팩터라고 정의한다. 예를 들어, 사람의 머리 색깔과 성별은 서로 무관 (또는 상대적으로 서로에 대한 영향이 적은)한 팩터들이다. 반면 성별과 헤어 스타일은 대체적으로 크게 correlate 되어있다. 각 팩터는 여러 값들을 가질 수 있으며, 같은 팩터에 속하는 값들은 남성과 여성, 금발 및 흑발과 같이 서로 disjoint하다. 각 데이터 샘플마다 존재하는 고유한 특성은 identity 팩터라고 정의한다.

%\subsection{Notation and Architecture}
%  Encoder \textbf{E}는 다음과 같이 입력 데이터 ${X}_{i}$를 입력받아 팩터 벡터 vector \textbf{c} 및 데이터 샘플 고유의 특징인 \textbf{z}으로 변환한다: $\textbf{c},\textbf{z} = \textbf{E}({X}_{i})$, \textbf{c}는 다음과 같이 여러 팩터 영역들로 나눠진다: $\textbf{c} =  \left[{c}_{1}, {c}_{2}, \cdots, {c}_{n}\right]$. 각 ${c}_{j}$는 특정 팩터에 대한 값을 갖게 된다. 이 중 우리가 바꾸고 싶은 팩터에 해당하는 부분만 원하는 값으로 바꿔준 뒤 decoder \textbf{G}에 넣으면 해당 팩터가 변한 새로운 데이터가 생성된다. 
%  학습 과정은 다음과 같다: 팩터 a의 값으로 a1을 가진 데이터를 입력으로 받아 \textbf{E}를 통해 za1를 만든다. 동시에 타겟 팩터 값 b1을 가진 데이터를 같은 방식으로 인코딩해 zb1을 만든다. za의 팩터 b 값을 b1으로 교체한 뒤 \textbf{G}를 이용해 새로운 데이터 $\textbf{x}_{new}$ 를 생성한다. 여기에 다음과 같은 2가지 loss를 부과한다.
  
    \begin{align}            
    L_{\!_{cons}} &= \frac{1}{N}\sum_{i=1}^{N}{\log\textbf{D}_{b}(\textbf{X}_{new})} \label{eq:gan_4}
%           L_{\!_{cons}} &= -\mathbb{E}_{x_{\!_A} \sim P_{\!_A}} \left[\log \textbf{D}_{b}(\textbf{X}_{new})\right] \label{eq:gan_4} 
    \end{align}
  

%\subsection{Factor Disentanglement}
  
%  An input data is expressed by set of latent features encoded by \textbf{E}, where specific elements of this features correspond to a factor. In Figure \ref{fig:figure_1}, we split this features into 3 pieces, and used the last piece as "hair color" factor. Factor entanglement process is conducted as follows: input images are sampled from the dataset, regardless of which domain they belong, and their latent features are encoded. At the same time, images of target domain are sampled, and also encoded into latent features. Then we change the piece of input features to that of target features, and then generate an image using the synthesized feature.  

==> text/model_v2.tex <==
\section{Model}

이 섹션에서는 universal translation을 위한 GeneGAN 구조를 제안하고, 이를 학습하기 위한 방법 및 이에 수반되는 문제들과 그에 대한 해결책을 제시한다. GeneGAN은 데이터를 genotype과 phenotype tensor로 인코딩하고, phenotype tensor의 여러 영역을 각 attribute에 임의로 할당한다. 변경하고 싶은 attribute 영역을 원하는 값으로 교체한 뒤 데이터를 재생성하면 해당 attribute가 "발현"된 데이터을 얻게 된다.  

  우리는 데이터를 이루는 일련의 특징들을 attribute ( or factor? )이라 부르며, 이 각 attribute가 가질수 있는 여러 값들을 attribute value라고 정의한다. 각 attribute들은 서로 independent하며, 같은 attribute에 속하는 value들은 서로 disjoint 하다고 가정한다. 예를 들어 사람의 얼굴 이미지는 머리 색깔 또는 성별 등의 attribute를 가질 수 있으며, 이 attribute들은 각각 금발과 흑발, 남성과 여성 등의 attribute value들을 가질 수 있다. 또한, 정의된 attribute를 제외한 나머지 모든 특징들은 각 데이터 샘플의 고유한 특징이라고 가정하며, attribut를 변경하더라도 이 부분은 변하지 않아야 한다. CrisphrGAN은 특정 데이터 샘플을 인코딩해 하나의 특징 tensor를 만들고, 각 attribute의 정보가 이 tensor의 특정 영역에 내장될 수 있다고 가정하며, 바꾸고 싶은 attribute 영역만 우리가 원하는 값으로 바꿔준 뒤 데이터를 재 생성할 수 있다.

%\subsection{Complex Translation}
%\input{text/complex_translation}

\begin{figure}[t]
  \begin{center}
  \centerline{\includegraphics[width=\linewidth]{Figures/Figure008_CRISPR_Cut_v_0_0_2_2017_05_18}}
  \caption{CRISPR CUT}
  \label{fig:complex_trans}
  \end{center}
\end{figure}

\begin{figure}[t]
  \begin{center}
  \centerline{\includegraphics[width=\textwidth]{Figures/Figure001_Main_Architecture_small_v_0_0_3_2017_05_17}}
  \caption{The architecture of GeneGAN}
  \label{fig:archi}
  \end{center}
\end{figure}


%\subsection{Composite Domain Distribution}
%\input{text/composite_domain_distribution}

% \begin{figure}[t]
%   \begin{center}
%   \centerline{\includegraphics[width=\textwidth]{Figures/CrisprGAN_archi4}}
%   \caption{The architecture of CrisprGAN}
%   \label{fig:archi}
%   \end{center}
% \end{figure}


\subsection{Architecture}

(To be replaced)\newline

As shown in Figure \ref{fig:archi}, GeneGAN has an Encoder $\textbf{E}$ a generator $\textbf{G}$, and a discriminator $\textbf{D}_{a}$ for each attribute $a$. 
GeneGAN 전체 구조는 그림 \ref{fig:archi}에 나타나 있듯이, encoder $\textbf{E}$와 decoder $\textbf{G}$를 각각 하나씩 갖고 있으며, 취급하려는 attribute 개수만큼의 discriminator $\textbf{D}_{a}$을 갖고 있다. Encoder E는 입력 이미지를 genotype 및 phenotype tensor로 인코딩하고, 바꾸고 싶은 target attribute의 이미지들로부터 genotype의 해 영역을 해당 attribute를 지닌 이미지들로부터 인코딩된 genotype tensor의 해당 attribute 부분 
% The architecture of CrisprGAN is shown in Figure \ref{fig:archi}. CriprGAN consists of three main components: (1) \textit{conversion-reversion autoencoder}, (2) \textit{conversion GANs} and (3) \textit{auxiliary autoencoder}. 

The conversion-reversion autoencoder is basically two stacked autoencoders: one for converted data generation and the other for reverted data generation.  The conversion-reversion autoencoder enables to learn the \textit{identify code} that captures the overall structure of data. 

The conversion GANs enable to learn the \textit{composable factor codes} \textit{c\textsubscript{i}} that capture partial attributes of data (e.g., the hair color of a face). As we mentioned in the introduction section, we explore to use GANs for discriminating a part of data instead of the full data. More formally, we use the discriminator to distinguish between conditioned data distribution $p_{data}(x|c_{i})$ and conditioned generation data distribution $p_{g}(x|c_{i})$. For his partial discrimination, we use simple but effective trick called \textit{factor conversion}. Through a minimax game, the disentangled factor code become more meaningful for the given factor.

Finally, the auxiliary autoencoder is used for factor conversion and reconstruction.

CrisprGAN has the identity code $z$ and can have $k$ factor codes $\{c_{1},c_{2},...,c_{k}\}$. However, for the convenience of explanation, we use only two factor codes $\{a,b\}$ in this section:
\begin{equation}
z \sim p_{z}, \quad a \sim p_{a}, \quad \textrm{and} \quad b \sim p_{b}
\end{equation}

We start by describing the conversion-reversion autoencoder. This mainly consists of two sub autoencoders: conversion autoencoder and reversion autoencoder. The conversion autoencoder takes data $x_{a,b}$ with the factors $a$ and $b$ as input, and generates partially converted data $x’_{a’,b}$. Here, $a'$ denotes factor conversion. The factor code $a$ to replace comes from the auxiliary autoencoder. It learns factored codes $\{z, a’, b\}$ by converting a factor code $a$. More formally, this can be described as follows:
\begin{equation}
E(x_{a,b}) = \{z, f_{a}(x_{a,b}), f_{b}(x_{a,b})\} = \{z, a, b\}
\end{equation}

Here, $f_{a}(x)$ denotes an encoding function that factors $a$ from $x$. Therefore, $f_{a}(x)=a$.
\begin{equation}
\textrm{factor conversion:} \quad a \rightarrow a'
\end{equation}
\begin{equation}
x'_{a',b} \sim p_{g}(x|z,a',b) = G(z, a', b)
\end{equation}

The reversion autoencoder takes sample data $x’_{a’,b}$ with the converted factor $a’$ as input, and generates reverted data $x''_{a,b}$ with the original factor $a$ and $b$. It learns factored codes $\{z, a, b\}$ by reverting a factor code $a$ (i.e., factor reversion). This can be formalized as follows:
\begin{equation}
E(x'_{a',b}) = \{z, f_{a}(x_{a',b}), f_{b}(x_{a',b})\} = \{z, a', b\}
\end{equation}
\begin{equation}
\textrm{factor reversion:} \quad a' \rightarrow a
\end{equation}
\begin{equation}
x''_{a,b} \sim p_{g}(x|z,a,b) = G(z, a, b)
\end{equation}

We note that the conversion autoencoder and reversion autoencoder share their parameters. More specifically, conversion encoder and reversion encoder share their parameters. Similarly, conversion decoder and reversion decoder do.

In CrisprGAN, the conversion GAN plays an important role. The generator $G$ of the conversion GAN takes the converted codes $\{z, a’, b\}$ as input, and generates a sample data $x’_{a’,b}$. The discriminator ${D_{a’}}$ of the conversion GAN takes a sample data ${x’_{a’,b}}$ and a real data $x_{a’,b}$ as input, and generates the probability that the sample data came from the real dataset. More formally, this can be described as follow:
\begin{equation}
D(G(z, a', b), x_{a',b}) = D(x'_{a',b},x_{a',b}) = p(real)
\end{equation}

The $G$ and $D$ are trained simultaneously in a way of a minimax game with the GAN objective $L_{D_{a’}}$. The objective will be explained in the next section.

%In addition to the conversion GAN, we can use a GAN for discriminating preserved factors. We call this auxiliary GAN as preservation GAN. The preservation GAN shares its generator $G$ with that of the conversion GAN. The discriminator $D_{b}$ of the preservation GAN takes a sample data $x_{a’,b}$ and a real data $x_{a,b}$ as input, and generates the probability that the sample data came from the real dataset. The $G$ and $D_{b}$ are trained simultaneously in a way of a minimax game with preservation GAN loss $L_{D_{b}}$.

\subsection{Multiplex Translation}
Each neural network of CrisprGAN can be jointly trained with backpropagation. The objective of CriprGAN consists of mainly three terms: (1) the conversion-reversion autoencoder objective for reconstruction, (2) the GAN objective for partial discrimination, and (3) the auxiliary autoencoder objective for reconstruction.

The conversion-reversion autoencoder has the following reconstruction objective: 
\begin{equation}
L_{RECON} = \mathbb{E}_{x \sim p_{data}(x), z \sim p_{z}}[||x_{a,b}-x''_{a,b}||_{2}]
\end{equation}

Here, we use $L_{2}$ loss, but $L_{1}$ may be used. It is known that $L_{2}$ loss generally results in blurry generation. However, since CrisprGAN has \textit{twisted} conversion-reversion autoencoder, the two options do not result in significant difference. This was also found in our previous work \cite{kim2017discogan}.

The conversion GAN has the following objective in the case of two factor codes $a$ and $b$:
\begin{equation}
L_{GAN_{conv}} = \mathbb{E}_{x_{a',b} \sim p_{data}(x_{a',b})}[\log D(x_{a',b})] + \mathbb{E}_{z \sim p_{z}(z)}[\log(1-D(G(z, a', b)))]
\end{equation}

The auxiliary autoencoder has the following reconstruction objective: 
\begin{equation}
L_{RECON_{2}} = \mathbb{E}_{x \sim p_{data}(x), z \sim p_{z}}[||x_{a',b}-x'_{a',b}||_{2}]
\end{equation}

Then, CrisprGAN has the following objective with hyperparameters $\alpha$, $\beta$, and $\gamma$:
\begin{equation}
L = \alpha L_{RECON} + \beta L_{GAN_{conv}} + \gamma L_{RECON_{2}}
\end{equation}

%\begin{equation}            
%L_{\!_{cons}} = \frac{1}{N}\sum_{i=1}^{N}{\log\textbf{D}_{b}(\textbf{X}_{new})} \label{eq:gan_4}
%\end{equation}

%\begin{equation}
%L_{\!_{cons}} = -\mathbb{E}_{x_{\!_A} \sim P_{\!_A}} \left[\log \textbf{D}_{b}(\textbf{X}_{new})\right] \label{eq:gan_4} 
%\end{equation}

==> text/model_v3.tex <==
\section{Reconfigurable Unpaired Image Translation}

\begin{figure}[t]
  \begin{center}
  \centerline{\includegraphics[width=0.8\linewidth]{Figures/Figure013_complex_im2im_translation_v_0_0_1_2017_05_19}}
  \caption{The motivation of reconfigurable image translation.}
  \label{fig:multiplex_concept}
  \end{center}
\end{figure}

We first provide the motivation for our work, formalize the problem and illustrate our proposed model and explain its components. We then explain the learning algorithm for our reconfigurable attribute translator.
%and finally propose an extension of our model for ``multiple translation'', in which multiple translations are simultaneously performed. 

%이 섹션에서는 먼저 논문에서 사용한 각종 개념 및 proposed GeneGAN을 정의하고, 어떻게 GeneGAN이 simplex translation task에 사용될 수 있는지 설명한다. 이후 multiplex translation으로의 확장에서 수반되는 문제점과, 이를 해결하기 위한 학습 scheme을 알려준다.

\subsection{Motivation}
%Fig 1a: naive approach
An image can be described in terms of many different attributes, where each attribute can take one of several values. For example, an image of a person may be described by attributes such as the gender, hair color and facial expression, each of which may take values such as male, brown, and smile, respectively. Then, the task of image translation can be viewed as changing the value of one or more attributes. 

Fig. \ref{fig:multiplex_concept}(a) illustrates all possible translations between images that are described using two attributes, each of which take one of two values, (A or B) and (X or Y) respectively. In the most naive approach, translating between all four image domains requires six separately trained translators (twelve if the translations are not bidirectional). 

%Fig 1b, 1c: smart approach. learn mapping for each attribute (single attribute translation)
In a more elegant approach, attribute-specific translators (e.g. mappings $G, G'$ and $F, F'$ in Fig. \ref{fig:multiplex_concept}(b, c)) can be learned instead to reduce the number of required translators. In such case, the sequential application single-attribute translators are sufficient to translate between all four image domains.  

%Our approach, even better, uses one reconfigurable translator network that can be readily changed to map between different domains
Our approach further simplifies the procedure by implicitly embedding multiple single-attribute translators into one reconfigurable translator network. By switching the desired target attribute values as needed, a single translator network can be used to translate images between multiple source-target domain pairs.   

\subsection{Formulation}

%Image representation, attributes 
We use the notation $a_{i,j}$ to denote that attribute $i$ (e.g. hair color) takes value $j$ (e.g. brown). If we suppose that there are $n$ attributes that describe an image dataset, each image $x$ can be represented using $n$ attributes and a sample specific feature $z$, where $z$ includes every information not related to any of $n$ attributes of our interest. 

% Domain, Translation as mapping between domains 
Also, we define an image domain as the set of all images that share one or more attributes values and an image translation as the mapping between two image domains. In the simplest case, an image translator $T$ can be viewed as a function that changes one attribute of the input image into a specific value. Often an image translator is rigid--it can only translated between two domains, and a separate translator must be trained for each source-target domain pairs. However, our translator is flexible--the desired target domain can be freely chosen for a single translator network without further training. 
\byoungjip{Please see whether "it can only translated" is correct in line 108.}

% Multiplex 
%In a more complex case, an image translator $T$ can simultaneously change more than one attributes into specific values, and we call this ``multiplex translation''.  Although In this work, we propose a reconfigurable multiplex image translation mechanism, where a single translator $T$ can be reconfigured by switching its desired target attributes as needed without further training. 

%   Image-to-image translation can be expressed as a mapping an image into a specific domain. We define a mapping function ${G(x,f_{ij})}$ that translates an image $x$ into an image of $j$th domain that belongs to $i$th attribute. The domain of $G$ is the complete set of images, and the range of it is its corresponding counterpart that belongs to domain: $G(x_{s}, f_{it}) = x_{t}$. In order to ensure 

% \subsection{Notation}
% A domain is defined as set of possible values of the independent variables, and a superdomain is the grouping of domains. An image can belong to one domain for each superdomain. For example, an image of human face can belong to "male" or "female" domain in "gender" superdomain. 

% An image can be expressed to have specific attribute values for each attributes, along with a sample-specific unique feature. We also define \textit{attribute code}, $f_{i}$, as the features of $i$th attribute, and each $f_{i}$ can have one of multiple values $v_{ij}$ depending on the number of possible attribute values of $i$th attribute. 

% From now on, we denote an image that belongs to 

% And then, to refer to an attribute value of an image (e.g., "man" and "woman"), we use the term \textit{attribute code}, and it is denoted by . An image can have $k$ attribute codes $\{f_{1},...,f_{k}\}$. Also, to refer to the codes that are not related to attribute codes, we use the term \textit{non-feature code}, and it is denoted by $z$.


  
\subsection{Components}

\begin{figure}[t]
  \begin{center}
  \centerline{\includegraphics[width=\textwidth]{Figures/Figure001_SIngle_Main_Architecture_small_v_0_0_5_2017_05_26}}
  \caption{The network architecture of proposed model. In this figure, we show an example of hair color attribute translation into "black hair". Input image is encoded into sample-specific feature $z$ and the characteristic attribute vectors $f$, where $f$ is split into multiple portions and allocated for each attribute. Hair color translation is done by replacing the corresponding attribute vector of the input image, $f_{3}$ by the target attribute vector $\bar{f_{3}}$, and the generator $G$ generates the translated image. Note that $\bar{f_{3}}$ is obtained by averaging $f_{3}$ of images having target attribute value (black hair). Sample specific feature $z'$ and characteristic attribute vectors $f'$ of the translated image is again encoded using $E$,  $f'_{i}$ is replaced by the original value, and back-translated image $x''$ is generated. This process is iterated for every attribute value $a_{i,j}$.\byoungjip{This caption is O.K, but it would be better to slightly revise.}} 
  \label{fig:archi}
  \end{center}
\end{figure}

Figure \ref{fig:archi} shows the overall architecture of our proposed model. It consists of two mapping functions (1) translator $T$ and (2) back-translator $T'$. From the model point of view, it has three distinct neural networks: an encoder $E$, a generator $G$, and a discriminator $D$ for each of the attribute value.%, and (3) associated adversarial discriminators $D$.

\paragraph{Translation.}
%(이걸 어떻게 표현할 지 모르겠는데, 이미지의 i번째 attribute를 j에서 k로 바꾸는 예를 여기에 보여주겠다...) 
Here, we illustrate the process of translating an input image $x$ into translated image $y'$ by changing its attribute $i$ to target value $k$ using translator $T$. First, an encoder $E$ encodes the input image $x$ into sample-specific feature $z$ and its characteristic attribute vector $f$, where $f$ is split into $n$ regions and each region is allocated for each attribute: $f_{i}$ denotes encoded vector of $i$th attribute for the input. The translator $T$ replaces $f_{i}$ of the encoded image into desired attribute value $f_{i,k}$, and the generator $G$ creates the translated image $y'$.  Note that $f_{i,k}$ indicates the encoded feature for attribute value $a_{i,k}$, and it is obtained by taking the average value of $f_{i}$ of images having attribute $a_{i,k}$. This process is shown in Figure \ref{fig:archi}. During training, we enforce the translated image to possess attribute value $a_{i,k}$ by using a discriminator that is specifically trained to discriminate on this attribute value. Note that, during the test phase, we can use either a target vector ($f_{i,j}$) obtained from averaging the vectors of all images with attribute value $a_{i,j}$, or a vector encoded from a specific instance. From this point, we denote the former case $translation$, and the latter $transfer$.

% . Note that $f_{i,j}$ indicates the encoded feature for attribute value $a_{i,j}$, and it is obtained by taking the average value of $f_{i}$ of images having attribute $a_{i,j}$

% \begin{equation}
% _{RECON} = \mathbb{E}_{x \sim p_{data}(x), z \sim p_{z}}[||x - x'||_{2}]
% \end{equation}
%The translation is expressed as a function $t : x \rightarrow y=T(x, v_{ik})$. 

% To map an input image $x$ into the output image $y$ in the target domain Y, the $G$ first   feature converter $C$ replaces source feature $f_{s}$ with a target feature value $v_{t}$. The target feature value $v_{t}$ is generated by encoding an image $x_{i}$ from a target domain $Y$ with the encoder $E$.

% \subparagraph{Adversarial Discrimination.}
% - Translation의  
% The adversarial discriminator $D_{Y}$ encourages translation function $t$ to generate output images $y_{i}$ indistinguishable from the real images from the target domain $Y$.

\paragraph{Back-translation.}
The sample specific feature $z$ and the values of non-target attributes must be retained during the translation process. In order to do so, translated image $y'$ is again encoded into sample-specific feature $z'$ and characteristic attributes $f'$. Now, $i$th attribute of $f'$ is replaced back to the original attribute value of the input $x$, $f_{i}$. The generator $G$ now generates a reconstructed image $x''$ from this attribute value. We enforce this reconstruct image $x''$ to match the original image as closely as possible. %This back-translation module leads
%rom generated translated $y'$ such that it matches the original input image $x$ as closely as possible. 

% - To maps an input image $y$ back to the source domain $X$, the feature converter $C$ replaces source feature $f_{s}$ with a source feature value $v_{s}$. Note that the translation function $t$ and back-translation function $t'$ share their parameters.

% Obejctive
\subsection{Objective}
 
Our model's objective is composed of two parts: an adversarial loss to ensure that target attributes are changed into desired values, and a reconstruction loss so that all other attributes and sample-specific features are retained. During the translation phase, the discriminator imposes following two losses: %generator $G$ and the discriminator $D$ receive following loss, respectively.

\begin{equation}
L_{GAN_{i,j}} = -\mathbb{E}_{y \sim p(y)}[\log D_{i,j}(y)] 
\end{equation}
\begin{equation}
L_{DIS_{i,j}} = -\mathbb{E}_{y \sim p(y)}[\log D_{i,j}(y)] - \mathbb{E}_{x \sim p_{data}(x)}[\log(1-D_{i,j}(y'))]
\end{equation}

during the back-translation phase, the distance between back-translated image $x''$ and the original input image, $d(x, x'')$ is minimized. This objective can be formally expressed as follows:
\begin{equation}
L_{RECON_{i,j}} = \mathbb{E}_{x \sim p_{data}(x)}[d(x, x'')]
\end{equation}

Any distance metric such as $L1$, $L2$ or Huber loss can be used for $d$. The final generation loss is now:
\begin{equation}
L_{GEN_{i,j}} = \alpha L_{RECON_{i,j}} + (1-\alpha) L_{GAN_{i,j}}
\end{equation}

The generation loss (6) is back-propagated to update the parameters of the encoder $E$ and the generator $G$, and the discriminator loss (4) is back-propagated to update parameters of the discriminator $D_{i,j}$ in rotation. For each iteration, above process is repeated for every attribute value $a_{i,j}$.


% \subsection{Training of Multiplex Translator}
% In addition to simple translation, translating one specific attribute of an image, our model can further perform multiplex image-to-image translation, which is a simultaneous translation of multiple attributes. While multiplex translation can be composed of simple translations, it requires sequential computations linear to the number of attributes to change. Since we perform translation simply by changing attribute codes inside the translator, changing multiple codes instead of one of them leads to simultaneous multiplex translation.

% However, training the model for simultaneous multiplex translation cannot be done easily. During training, the most intuitive method to train multiplex translator is using multiple discriminator at the same time. For example, if we want to translate an image of male with black hair into a female with blond hair, we can apply two discriminator $D_{blond}$ and $D_{female}$ at the same time. The distribution matching ability of generative adversarial networks (GANs) make this approach infeasible. The domain of images of blond hair consists uniformly distributed male and female images, and $D_{blond}$ expects $G$ to generate images of both male and female with blond hair. On the other hand, the domain of female images contain images with many hair colors, therefore $D_{female}$ enforces $G$ to generate female images with both black and blond hair. Since those two discriminators' objective contradict each other, $G$ fails to create intended images, as depicted in Figure \ref{fig:multiplex_solve}. 

% In order to resolve this, we designed a training technique suited for multiplex translation. Instead of applying $D_{blond}$ and $D_{female}$ simultaneously, we use one of them sequentially. When applying generated female images with blond hair to $D_{blond}$, we additionally generate images of blond hair



% \begin{figure}[t]
%   \begin{center}
%   \centerline{\includegraphics[width=\textwidth]{Figures/Figure003_Complex_translation_Sampling_Converting_v_0_0_1_2017_05_17}}
%   \caption{To solve Multiplex Image-to-Image Translation }
%   \label{fig:multiplex_solve}
%   \end{center}
% \end{figure}



==> text/todo.tex <==
\section{TODO}
\subsection{꼭 해야할 일}
\begin{enumerate}
\item Abs. rewrite
\item Intro rewrite
\item Fig 1 생성
\item Model 설명 클리어하게 
\end{enumerate}
\subsection{체크 또는 고민할일}
\begin{enumerate}
\item DiscoGAN으로 baseline 만들것인지..?
\item icgan과의 차이점?
\end{enumerate}
